Reward Finetuning for Faster and More Accurate Unsupervised Object Discovery

Recent advances in machine learning have shown that Reinforcement Learning from Human Feedback (RLHF) can improve machine learning models and align them with human preferences. Although very successful for Large Language Models (LLMs), these advancements have not had a comparable impact in research for autonomous vehicles -- where alignment with human expectations can be imperative. In this paper, we propose to adapt similar RL-based methods to unsupervised object discovery, i.e. learning to detect objects from LiDAR points without any training labels. Instead of labels, we use simple heuristics to mimic human feedback. More explicitly, we combine multiple heuristics into a simple reward function that positively correlates its score with bounding box accuracy, i.e., boxes containing objects are scored higher than those without. We start from the detector's own predictions to explore the space and reinforce boxes with high rewards through gradient updates. Empirically, we demonstrate that our approach is not only more accurate, but also orders of magnitudes faster to train compared to prior works on object discovery.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/explore-fg.tex <==
\begin{table}[ht]
\begin{tabular}{@{}llcclcccc@{}}
\toprule
                              &  & \multicolumn{2}{c}{Recall} &  & \multicolumn{4}{c}{mAP IoU 0.7}     \\ \cmidrule(lr){3-4} \cmidrule(l){6-9}
                        Explor. Strategy      &  & IoU 0.1      & IoU 0.7     &  & 0 - 30 & 30 - 50 & 50 - 80 & 0 - 80 \\ \midrule 
Sample near pred. (30 ep)     &  & 61.2         & 26.1        &  & 33.0   & 18.9    & 1.8     & 18.9   \\
~~~+ near foreground &  & 73.1         & 23.6        &  & 17.9   & 15.6    & 1.4     & 12.0   \\ \midrule
Sample near pred. (60 ep)     &  & 76.2         & 30.3        &  & 38.4   & 23.9    & 3.3     & 22.8   \\
~~~+ near foreground &  & 75.8         & 30.0        &  & 39.1   & 22.8    & 3.2     & 22.6   \\ \bottomrule
\end{tabular}
\caption{Exploration near predictions or with exploration at foreground proposals. Observe that sampling near foreground increases the recall (30 epochs). This advantage is not prominent at higher training epochs as the model's own generalization improves.}
\label{tab:explore-fg}
\end{table}

==> tables/ithaca-updated.tex <==
\begin{table}[h]
\captionsetup{aboveskip=7pt}
\centering
\caption{\textbf{Detection performance on Ithaca365.} This table corresponds with Table 2 of the main paper, with the Self-Training baseline updated to include 300 epochs.}
\label{tab:ithaca-updated}
\begin{tabular}{@{}llcccclccc@{}}
\toprule
                                               &  & \multicolumn{4}{c}{mAP @ 1m ($\uparrow$)} &  & \multicolumn{3}{c}{Errors 0-80m ($\downarrow$)} \\ \cmidrule(lr){3-6} \cmidrule(l){8-10} 
\multirow{-2}{*}{Method}                       &  & 0-30     & 30-50     & 50-80    & 0-80    &  & ATE            & ASE            & AOE           \\ \midrule
No Finetuning                                  &  & 18.7     & 4.8       & 0.0      & 7.7     &  & 1.17           & 0.60           & 1.64          \\
Self-Train. (30 ep)                            &  & 25.9     & 9.2       & 1.2      & 12.4    &  & 1.08           & 0.62           & 1.57          \\
\textbf{Self-Train. (300 ep) }                          &  & 16.3     & 3.6       & 1.8      & 6.8     &  & 1.19           & 0.74           & 1.57          \\
MODEST (30 ep)                                 &  & 14.6     & 0.7       & 0.0      & 3.7     &  & 0.83           & 0.52           & 1.53          \\
MODEST (300 ep)                                &  & 27.5     & 26.3      & 21.0     & 27.1    &  & 1.06           & 0.67           & 1.09          \\
DRIFT (15ep)                                   &  & 39.1     & 24.3      & 17.7     & 28.0    &  & 0.73           & 0.33           & 1.23          \\
DRIFT (30 ep)                                  &  & 47.1     & 31.2      & 22.9     & 35.1    &  & 0.49           & 0.35           & 1.20          \\
{\color[HTML]{999999} Sup. on KITTI}           &  & 59.8     & 28.3      & 4.0      & 32.0    &  & 0.26           & 0.22           & 0.46          \\
{\color[HTML]{999999} Sup. on Ith365 (in dom)} &  & 75.7     & 48.3      & 22.6     & 51.5    &  & 18.0           & 12.9           & 33.0          \\ \bottomrule
\end{tabular}
\end{table}

==> tables/per_class.tex <==
\begin{table}[h]

 \begin{subtable}[h]{\linewidth}
\begin{tabular}{@{}llccccccccc@{}}
 \toprule 
    & &    \multicolumn{4}{c}{mAP IoU 0.5} & & \multicolumn{4}{c}{mAP IoU 0.7}\\
     \midrule &
      & 0-30        & 30-50        & 50-80        & 0-80      &  & 0-30        & 30-50        & 50-80        & 0-80        \\\cmidrule(lr){3-6} \cmidrule(l){8-11} 
MODEST &  & 65.4        & 50.2         & 10.7         & 43.9        & & 47.7        & 20.7         & 2.1          & 24.6        \\
ST    & & 63.1        & 41.7         & 6.4          & 38.8     &   & 45.6        & 14.6         & 0.6          & 21.9        \\
\ours{}  & & 70.3 & 60.1 & 20.3 & 52.7 &  & 57.6 & 42.9 & 8.3 & 38.2     \\\bottomrule
\end{tabular}
\caption{Car}
\end{subtable}
\hfill
\begin{subtable}[h]{\linewidth}
 \begin{tabular}{@{}llccccccccc@{}}
 \toprule 
    & &    \multicolumn{4}{c}{mAP IoU 0.5} & & \multicolumn{4}{c}{mAP IoU 0.7}\\
     \midrule &
      & 0-30        & 30-50        & 50-80        & 0-80      &  & 0-30        & 30-50        & 50-80        & 0-80        \\\cmidrule(lr){3-6} \cmidrule(l){8-11} 
MODEST &  & 7.5                                              & 3.9                                              & 0.3                                            & 3.7                                              &  & 1.9          & 1.2          & 0.3         & 1.1       \\
ST    & & 5.5                                              & 0.8                                              & 0                                              & 2                                                & & 1.4          & 0.3          & 0           & 0.5        \\
\ours{}  & & 8.9 & 2.8 & 0.2 & 3.6 &  & 4.3 & 1.3 & 0.1 & 1.8      \\\bottomrule
\end{tabular}
\caption{Pedestrian}
\end{subtable}

\begin{subtable}[h]{\linewidth}
\begin{tabular}{@{}llccccccccc@{}}
 \toprule 
    & &    \multicolumn{4}{c}{mAP IoU 0.5} & & \multicolumn{4}{c}{mAP IoU 0.7}\\
     \midrule &
      & 0-30        & 30-50        & 50-80        & 0-80      &  & 0-30        & 30-50        & 50-80        & 0-80        \\\cmidrule(lr){3-6} \cmidrule(l){8-11} 
MODEST &  & 10.5                     & 0.2                       & 0                         & 3.6                      & & 6.7  & 0.1   & 0     & 2.2     \\
ST    & & 7.5                      & 0.1                       & 0                         & 2.6                      & & 4.7  & 0     & 0     & 1.4   \\
\ours{}  & & 46.1 & 6.1 & 0.2 & 22.2 &  & 33.9 & 0.6 & 0 & 14.2      \\\bottomrule
\end{tabular}
\caption{Cyclist}
\end{subtable}
\begin{subtable}[h]{\linewidth}
 \begin{tabular}{@{}llccccccccc@{}}
 \toprule 
    & &    \multicolumn{4}{c}{mAP IoU 0.5} & & \multicolumn{4}{c}{mAP IoU 0.7}\\
     \midrule &
      & 0-30        & 30-50        & 50-80        & 0-80      &  & 0-30        & 30-50        & 50-80        & 0-80        \\\cmidrule(lr){3-6} \cmidrule(l){8-11} 
MODEST &  & 17.9                     & 8.4                       & 0.5                       & 9.9                      &  & 6.2  & 1.6   & 0.6   & 1.9      \\
ST    & & 18.3                     & 8.5                       & 0.1                       & 7.5                      &  & 7.8  & 0.9   & 0.1   & 1.5     \\
\ours{}  & &  37.3 & 13.8 & 0.7 & 16.3 &  & 12.5 & 2.4 & 0.1 & 3.5   \\\bottomrule
\end{tabular}
\caption{Truck}
\end{subtable}

\caption{BEV mAP per Class}
\end{table}

==> tables/search-seeds.tex <==
\begin{table}[h]
\centering
\caption{Search boxes from the reward function.}
\label{tab:search}
\begin{tabular}{@{}llcccclcccc@{}}
\toprule
                  &  & \multicolumn{4}{c}{mAP IoU 0.5} &  & \multicolumn{4}{c}{mAP IoU 0.7} \\ \cmidrule(lr){3-6} \cmidrule(l){8-11} 
                  &  & 0-30  & 30-50  & 50-80  & 0-80  &  & 0-30  & 30-50  & 50-80  & 0-80  \\ \midrule
MODEST Seeds      &  & 25.1  & 5.8    & 0.8    & 8.8   &  & 12.9  & 1.2    & 0.1    & 3.5   \\
Searched Boxes    &  & 11.7  & 7.4    & 4.0    & 7.1   &  & 4.2   & 2.1    & 0.7    & 2.0   \\
Train on seed     &  & 44.1  & 21.1   & 1.2    & 23.9  &  & 24.4  & 6.0    & 0.1    & 10.5  \\
Train with search &  & 35.3  & 26.3   & 11.7   & 25.3  &  & 29.6  & 21.2   & 6.7    & 20.1  \\ \bottomrule
\end{tabular}
\end{table}
